Arm Robot: AR-Enhanced Embodied Control and Visualization for Intuitive Robot Arm Manipulation

Embodied interaction has been introduced to human-robot interaction (HRI) as a type of teleoperation, in which users control robot arms with bodily action via handheld controllers or haptic gloves. Embodied teleoperation has made robot control intuitive to non-technical users, but differences between humans' and robots' capabilities \eg ranges of motion and response time, remain challenging. In response, we present Arm Robot, an embodied robot arm teleoperation system that helps users tackle human-robot discrepancies. Specifically, Arm Robot (1) includes AR visualization as real-time feedback on temporal and spatial discrepancies, and (2) allows users to change observing perspectives and expand action space. We conducted a user study (N=18) to investigate the usability of the Arm Robot and learn how users perceive the embodiment. Our results show users could use Arm Robot's features to effectively control the robot arm, providing insights for continued work in embodied HRI.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> chapters/3_design_old.tex <==
\section{Interaction Design}
\label{design}

In this section, we describe the design goals of Arm Robot, and elaborate the design in two folds: embodied control and visualization. 

\subsection{Design Goals}
The overarching goal of Arm Robot is to help users handle the human-robot differences in ranges of motion and response time.

The concrete design goals are as follows,

\begin{itemize}[nosep,leftmargin=*]
    \item \textbf{DG1:} Allow users to embody the robot arm with free hand.
    \item \textbf{DG2:} Augment users' perception of discrepancies in ranges of motion and response time.
    \item \textbf{DG3:} Extend or compress users' ranges of motion with flexible spatial mapping.
\end{itemize}

\subsection{DG1: Freehand Embodied Teleoperation}
% Metaphors are the key concept of interaction design, especially for embodied interaction. Table \ref{tab:embodied_metaphors} depicts the metaphors we used in embodied control.

Arm Robot's interaction centers on freehand embodiment, using the ``gripper as hand'' metaphor. Wrist movements are mirrored by the robot's gripper in 6-DOF, including grasping actions.

% The core interaction of Arm Robot is freehand embodied teleoperation. The metaphor is ``gripper is hand''. When one translates or rotates their wrist, the base of the robot gripper imitates the 6-DOF pose. When one's fingers close to "grasp", the robot gripper also grasps. 

\subsection{DG2: Augment Perception of Discrepancies}

We display two digital twins rather than abstract text to augment user perception with visual feedback. 

In specific, Arm Robot includes two digital twins.

The first digital twin is a full robot arm superposed right on the physical one. The digital twin shows the robot's motion without delay in AR. In other words, it is the zero-delay version of the physical robot. This digital twin is made translucent to avoid any visual occlusion of the real robot. When the real robot arrives at the target pose indicated by the virtual robot, they will fully overlap. This intends to augment users' perception of different response time. 

This virtual robot also changes color from translucent white to bright orange when the intended motion is impossible due to robot kinematics. For example, if a user continuously moves in a direction and goes beyond the range of the robot's motion, the robot will turn orange as an anomaly signal. This feature aims to augment users' perception of different ranges of motion.

The second digital twin is a virtual gripper that overlaps with the embodying hand. The virtual gripper is translucent so users can still see their hand through the gripper. This visualization gives users an idea of the correspondence between their hand and the robot gripper.

\subsection{DG3: Adjustable Spatial Mapping}

We adopted the absolute coordination system to track hand position. The human hand's range of motion can be extended by walking or bending. But this is not enough. 

We augmented users' range of motion through three interactions to change the spatial mapping between the hand and the gripper. They are the on/off switch, the scale of mapping, and the mirror reversal of mapping. Note that we recommend turning off embodiment to free the hand for other operations like scaling or mirroring. 

\subsubsection{``Freeze/Unfreeze''}
We connected a line between the wrist and the physical gripper. When the line is green, the embodiment is on. Users can use the other hand to pinch the line. After the pinch, the line will turn grey indicating that the embodiment is paused. We call it ``Freeze''. Once the gripper freezes, users can freely move to another position while the positional offset of spatial mapping keeps updated with the new relative position between the hand and the gripper. The new spatial mapping will take effect after the user pinches the line to unfreeze the gripper.

% Users can extend their range of motion with this ``freeze - move - unfreeze'' interaction. Suppose one wants to move the gripper upwards to the robot extreme. In such a case, the user can first move the gripper to the highest possible position by fully extending their arm up via teleoperation. Then, they freeze the gripper there and move their hand from above their head back to chest level, which updates the spatial mapping between hand and gripper. When resuming teleoperation, the new spatial mapping takes effect and allows controlling the gripper above the initially reachable space by moving their hand from chest to overhead again. This technique extends the user's effective range without requiring exaggerated body movements like standing on a chair. 

\subsubsection{``Scale''}

Users can modify the scale of spatial mapping by interacting with a disk. They can resize the disk with two-hand manipulation. The disk radius indicates the ratio of robot motion to hand motion. For example, if the disk is resized as twice as large, one inch of hand movement will become two inches of gripper movement. The disk can be shrunk to half or enlarged to double. This feature is called ``Scale''.

This feature was designed to augment or shrink effective human motion range to adapt to the robot workspace.

\subsubsection{``Mirror''}

Mirror reversal of motion is designed as an alternative spatial mapping to fit into the motion range when the target object is between the operator and the robot. We place two solid arrows embodying the X and Y axes on the disk. Users can rotate an arrowhead 180 degrees to reverse the robot's motion on that axis. 

For example, when users approach the robot along this axis in ``Mirror'' mode, the robot will approach the users too, instead of shifting away in the same direction. The robot imitates the moves seemingly as the user's reflection in the mirror.



% We came up with these interactions by heuristics and common sense, knowing that they are not the exclusive designs to satisfy the design requirements.

% the chart of metaphor-virtual action-physical action: Eliciting Embodied Metaphors through Augmented-Reality Game Design

\begin{table}[htp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{2cm}p{3cm}p{3cm}@{}}
    \noalign{\hrule height 1pt}  
         \textbf{Metaphor} & \textbf{Virtual Action} & \textbf{Physical Action} \\
    \noalign{\hrule height 1pt}  
    \multirow{2}{*}{\textbf{Gripper is hand}} & Rotate and translate the gripper & Rotate and translate the embodying hand\\
     & Gripper grasps & Hand grasps \\
    \noalign{\hrule height 1pt}  
    Embodiment toggle is line & Pause/Resume embodiment & Pinch the line to switch between grey/green \\
    \midrule
    Scale is disk & Scale up/down the gripper translation & Drag the disk with two hands to resize it\\
    
    \midrule
    Coordinate axes are arrows & Reverse robot motion on the axis & Flip an arrow \\
    
    
    \noalign{\hrule height 1pt}  
         
    \end{tabular}}
    \caption{Metaphors, virtual actions, and physical actions of embodied interactions in Arm Robot.}
    \Description{
    This table presents metaphors for embodied interactions in Arm Robot, with corresponding virtual and physical actions. The “Gripper is hand” metaphor equates rotating and translating the gripper with similar hand movements and associates the gripper's grasp with the hand's grasp. “Embodiment toggle is line” metaphor links pausing and resuming the embodiment to pinching a line that toggles color from grey to green. The “Scale is disk” metaphor relates scaling the gripper's movement to dragging a two-handed disk to resize. Lastly, the “Coordinate axes are arrows” metaphor connects reversing the robot's axis motion to flipping an arrow. 
    }
    \label{tab:embodied_metaphors}    
\end{table}


==> chapters/8_limitation.tex <==

\subsection{Depth Perception}
%common problem with depth perception, especially from the side perspective as opposed to the front-on perspective. %
Given the nature of passthrough mode, where the real world is captured by cameras in front of the headset and projected using the two screens in the headset, users experience a similar perspective of what they would see using their own eyes. However, the projection is not a perfect recreation of human eyesight due to misaligned cameras and digital restraints in the screens. The former refers to the fact that the camera is not at the same height of what the user is accustomed to, while the latter refers to warping near the edges of the screen as well as their digital resolution. Due to these limitations, we found that users experienced a decrease in their depth perception. In our user study, the majority of our participants preferred standing in front of the robot arm as opposed to the side or behind. This is likely due to the layout of the table as shown in Figure \ref{fig:floorplan}. The frontal view only needs accurate depth perception between the target and the robot's base, whereas the side view needs the accurate depth perception for the length of the table. Future work should aim to maintain an equal distance between the robot base and the user's position to ensure that depth perception is similar in both perspective. In addition to this, future improvements in hardware capabilities may also alleviate this issue.

% P12 The further you are away, the more difficult it is to control (depth perception is off) ``even though the VR robot is directly above the cube, the real robot is off. However, when you are close, the error is much closer.''

% p16 - Hard to tell the depth of the table but the horizontal movement is easy. Since they use their hand in a forward orientation, it sometimes occludes the gripper when moving and difficult to tell depth

% \subsection{Balance between Manual Control and Automation}
%dynamic scaling

% \subsection{Rotation Offset}
% How to allow rotation offset while keeping the sense of embodiment is still a challenge. we did not solve it quite well. More investigation into this


% Majority of our participants preferred front view
%front view offers better idea of the surface but that may be due to how narrow the table is on the side (less room for error in the front since you can only miss by small length, whereas the side view, you can miss by the entire length of the table almost)

%preferred front view but also used side view to avoid collision the robot itself
%side view used to check if the gripper was in the correct position to grab the object
%standing to the side could also have the opposite effect of blocking the object
% side view was better at gauging where objects were since the user could "see" it from the robot's perspective

% \subsection{Force Feedback} 
% Whether the force is big enough to grasp, or whether the force is small enough for gentle manipulation, what is the texture (hard/soft/rough/smooth) to tell the status of the object (e.g., flour, vulnerability)
% 


% \subsection{Precision} 
%Our robot is not the most stable possible.
% hand tracking shake too. can be fixed with a low-pass filter, but that will introduce more lag
